The Trade-off between Universality and Label Efficiency of Representations from Contrastive Learning

Pre-training representations (a.k.a. foundation models) has recently become a prevalent learning paradigm, where one first pre-trains a representation using large-scale unlabeled data, and then learns simple predictors on top of the representation using small labeled data from the downstream tasks. There are two key desiderata for the representation: label efficiency (the ability to learn an accurate classifier on top of the representation with a small amount of labeled data) and universality (usefulness across a wide range of downstream tasks). In this paper, we focus on one of the most popular instantiations of this paradigm: contrastive learning with linear probing, i.e., learning a linear predictor on the representation pre-trained by contrastive learning. We show that there exists a trade-off between the two desiderata so that one may not be able to achieve both simultaneously. Specifically, we provide analysis using a theoretical data model and show that, while more diverse pre-training data result in more diverse features for different tasks (improving universality), it puts less emphasis on task-specific features, giving rise to larger sample complexity for down-stream supervised tasks, and thus worse prediction performance. Guided by this analysis, we propose a contrastive regularization method to improve the trade-off. We validate our analysis and method empirically with systematic experiments using real-world datasets and foundation models.

==> 9_plan.tex <==
% \subsection{Experiments List}
% \begin{enumerate}
%     \item Trade off exists
%     \begin{itemize}
%         \item Trade-off vs Universality: [MoCo v2, SimSiam, NNCLR] tested on [CIFAR10, MNIST, Fer2013] for 4 datasets
%     \end{itemize}
%     \item Property 
%     \begin{itemize}
%         \item Quantitative study: Similarity
%         \item Ablation study
%         \begin{itemize}
%             \item Replacing CINIC-10 With CIFAR-10 for [MoCo v2, SimSiam]
%             \item Varying Target-Relevant pre-training Data Percentage [MoCo v2, SimSiam]
%             \item Varying the Class Number of ImageNet32 [MoCo v2, SimSiam]
%         \end{itemize}
%     \end{itemize}
%     \item Solution
%     \begin{itemize}
%         \item Fine-tune
%         \item Qualitative study: Cluster Visualization
%         \begin{itemize}
%             \item CLIP
%             \item MoCo V3
%             \item SimCSE
%         \end{itemize}
%     \end{itemize}
% \end{enumerate}

\section{Plan}

\YL{
\begin{enumerate}
    \item Basic experiments demonstrating the trade-off.
    \begin{enumerate}
        \item Suggestions: aiming for the following figure: 
        x-axis corresponds to (1) pretrained on CINIC10, (2) CINIC10+SVHN, (3) CINIC10+SVHN+GTSRB, (4) CINIC10+SVHN+GTSRB+part 1 of ImageNet, (5) CINIC10+SVHN+GTSRB+part 1 and part 2 of ImageNet, etc. 
        x-location depends on the number of unlabeled data used. 
        y-axis corresponds to the test accuracy on CIFAR10 trained with certain amount of labeled data. Can have a curve for each value of the amount of labeled data used. 
        \item Dimensions: 1) different methods: SimSiam, MoCo, Barlow Twins etc; 2) different datasets: outside the CIFAR10 setting, we can consider the MNIST setting: pretrain EMNIST and then mixed with other digits datasets, test on MNIST. STL10 can also be considered but need more careful investigation since it's different from MNIST and CIFAR10, ie, it has labeled and  unlabeled data while the unlabeled is not from the same distribution as the labeled data, but from ImageNet. STL10 can be combined with subsets of ImageNet for pre-training. 
    \end{enumerate}
    \item Ablation experiments investigating the conditions of the trade-off: when the unlabeled data for the specific task is large, adding diverse other datasets brings more negative impact than positive benefits (that will pack too much information not related to the specific task but will not add much information related).   
    \begin{enumerate}
        \item Varying the unlabeled data size related to the specific task. E.g., do experiments for different percentage p on (1) p\% of CINIC10, (2) (p\% of CINIC10)+SVHN, (3) (p\% of CINIC10)+SVHN+GTSRB, (4) (p\% of CINIC10)+SVHN+GTSRB+part 1 of ImageNet, (5) (p\% of CINIC10)+SVHN+GTSRB+part 1 and part 2 of ImageNet, etc.
        \item Varying the labeled training data size (already done above in the demonstrating the trade-off). Plot the figure: x-axis is the labeled training data size, y-axis is the test accuracy, each curve corresponds to a different set of pretraining datasets. This is to show that: when pretraining on diverse datasets (most of) the info useful for the specific task is still in the representation (not washed out by the other dissimilar datasets), but needs more labeled data to pick up. The fact that the info is still there gives justification of possibility to improve the prediction performance on universal representations (i.e. the next set of experiments).
    \end{enumerate}
    \item Algorithm design to improve the trade-off. Dimensions to consider:
    \begin{enumerate}
        \item What are the inputs? Using only the limited labeled data from the target task or limited labeled data + some unlabeled data from the target task?
        \item Whether the pre-trained model can be fine-tuned? Allowed to fine-tune or just to train the linear classifier? 
    \end{enumerate}
\end{enumerate}
}



\ZS{One proposal for the third point, which is about three steps training. 
\begin{itemize}
    \item (I) The foundation model trained on $n_1$ \textbf{unlabeled} data points (may from many diverse domains) by contrastive learning.
    \item (II) For the downstream task, use $n_2$ \textbf{unlabeled} data from the target task to "Fine-tune" the foundation model by contrastive learning with some \textbf{regularization} effect, where $n_2<<n_1$.
    \item (III) Finally, use $n_3$ \textbf{labeled} data from the target task to supervised train the linear classifier, where $n_3 << n_2$. 
\end{itemize}  
}

\ZS{
\begin{enumerate}
    \item Due to universality, the model trained by (I) only need to do feature "selection" in step (II) and no need to do long time optimization to learn features. If we skip step (I), we need much larger $n_2$ and much longer unsupervised training time to learn features.
    \item For label efficiency, in step (III), the model trained by step (I) + (II) may use much fewer samples (smaller $n_3$) to beat the model trained with step (I) only.
    \item The three steps training makes sense under this assumption. The diverse domains training data in step (I) is very cheap. The unlabeled task data in step (II) is expensive but still much cheaper than labeled task data in step (III). 
    \item We need to consider or compare with supervised Finetune by labeled task data. Note that in the above proposal, we do not have supervised Finetune and we only have supervised Linear Probing. May consider OOD effect here.
\end{enumerate}
}

\EL{An idea about the (II) of Zhenmei's proposal above, which is about the 'fine-tune' process after pre-training.
\begin{enumerate}
    \item For supervised fine-tune process instead of the unsupervised one described in (II) , we could use self-distillation to alleviate catastrophic forgetting on the pre-trained representation (which might lead to low accuracy while having more data points in pre-training in our experiment). [reference: \href{https://arxiv.org/abs/2205.00506}{Preserve Pre-trained Knowledge: Transfer Learning With Self-distillation For Action Recognition}]
    \item Specifically, we could have a teacher model (i.e., a copy of the representation from last epoch (as mentioned in the reference paper) OR a representation generated with a momentum encoder). Then start the self-distillation process with the teacher model and the current representation (i.e., calculate the Euclidean distance between the two encoders as the loss function). 
    \item Treat the self-distillation as a regularization term and combine it with the loss from supervised contrastive learning to calculate the total loss.
    \item Similar process might also be adapted in unsupervised setting of the fine-tune process mentioned in (II) to preserve more knowledge of the representation got from pre-training.
    
\end{enumerate}

}

==> script/bar_main.tex <==

% \begin{figure}[ht!]
%     \centering
%     \newcommand{\imagewidth}{0.32\linewidth}
%     {\includegraphics[width=\imagewidth]{figure/bar/CLIP_10.pdf}}
%     {\includegraphics[width=\imagewidth]{figure/bar/MOCO_V3_10.pdf}}
%     {\includegraphics[width=\imagewidth]{figure/bar/SIMCSE_10.pdf}}
%     \caption{\ZS{TODO} \YL{The figures do not seem to show good advantages of our method. Maybe we should have a table of 3 column blocks (corresponding to 3 pretrained models); in each column block, the columns correspond to the target tasks; the rows are LP/FT/Ours; highlight the best results in each column. } }
%     \label{fig:bar_main}
% \end{figure}
